Research in Visible Light Communication Systems with OpenVLC1.3

In this paper, we present the design and implementation of our latest OpenVLC1.3 platform to perform research in Visible Light Communication Systems. We retain the advantages of the previous versions such as TCP/IP layers support, software programmability and low-cost front-end. We re-design the transceiver to support higher modulation rates and sensitivity. This allows us to reach a throughput of 400 kb/s (a factor of 4 with respect to the previous version) and increase the distance by a factor of 3.5. We further improve the software robustness of the system and reduce the form factor at similar hardware cost.

==> sec/acknowledgements.tex <==

\section*{Acknowledgment} \label{sec_acknowledgements}

This work has been funded in part by the Madrid Regional Government through TIGRE5-CM (S2013/ICE-2919)
and in part by the ``La Caixa international PhD program'' fellowship.

==> sec/background.tex <==
\section{Background} \label{sec_background}
\note[DG]{remove or rewrite}
\subsection{Earlier versions of OpenVLC}
The previous versions of 
OpenVLC mainly consisted of three parts: the BeagleBone Black board~\cite{BBB}, the cape, and the driver.
\begin{itemize}
	\item \emph{BeagleBone Black (BBB):} a low-cost embedded platform ($\approx$55 USD) that runs Linux Operating 
System, equipped with a AM335x 1\,GHz CPU, two Programmable Real-time Units (PRUs), and 65 GPIOs for quick prototyping.
	\item \emph{OpenVLC cape:} the front-end transceiver that is attached directly to the BBB. The cape is equipped with one 
high-power LED, one low-power LED and one photodiode. Depending on the application scenario, either the high-power LED or the low-power LED can be configured as the transmitter. The low-end LED can also be configured as a receiver to detect incoming light signals. 
	\item \emph{OpenVLC driver:} the implementations of VLC MAC and PHY layers in the Linux kernel. The key primitives are sampling, 
	symbol detection, coding/decoding, channel contention, carrier sensing and Internet protocol interoperability.
\end{itemize}


\subsection{PRUs of the BBB}

The PRUs are exploited in this work to control the hardware more precisely and faster. A PRU is a fast processor operating at 
200\,MHz with 32-bit registers.
 It has single-cycle input/output access to a set of BBB pins and peripherals, and can access the 
memory shared by the CPU of BBB. %The architecture of PRU SoC is shown in Figure~\ref{fig_pru_block}.
The PRUs are programmed in assembly with a limited set of instructions. This makes programming 
them difficult, but allows to have a tight timing control over the hardware. 

% 
% \begin{figure}[b]
% 	\centering
% 	\includegraphics[width=.9\columnwidth]{figures/PRU_SoC}
% 	\caption{PRU System-on-Chip architecture~\cite{PRU_development}.}
% 	\label{fig_pru_block}
% \end{figure}





==> sec/cape.tex <==
%\section{Cape} \label{sec_cape}



==> sec/discussion.tex <==
\section{Discussion}

%\comment[Qing]{We need to discuss the applications that can be enabled by OpenVLC1.2, esp. applications related to on-demand networking systems}
To the best of our knowledge, OpenVLC is the first open platform that reaches 100 Kbps using VLC. Nevertheless, there is a long way to go. We are currently working on making OpenVLC 1.2 bi-directional, interface it with more powerful lights and increasing the throughput even more. This platform could then be used not only for research and teaching, but also to create real world applications. Because artificial light is almost anywhere in our lives, OpenVLC could be used in applications from museum audio touring to vehicular road congestion detection or even patient monitoring and tracking in hospitals. 

==> sec/driver.tex <==


%Although the PRUs only allow TX 
%or RX (in the current implementation, not at the same time), the kernel allows both TX and RX at the same time, providing two 
%advantages:

%\begin{itemize}
%	\item If the code of the PRU is modified transmission and reception could be perform at the same time (limiting the 
%throughput and accuracy).
%	\item In future releases of BBB, if more PRUs are installed, this would allow an easy adaptation for full-duplex 
%transmission.
%\end{itemize} 


 
 





==> sec/firmware_interface.tex <==










==> sec/hardware.tex <==
%\section{Hardware differences}
\section{OpenVLC1.2 Cape}
\comment[Qing]{Assigned to Qing.}

The OpenVLC board also has been modified to meet the needed requirements. It is based in the previous version of the board (\textcolor{red}{add ref}) and several modifications have been done. Although the board is unique, it is divided into two parts, the TX and RX circuits.

\begin{figure}[t]
	\centering
	\includegraphics[width=.4\columnwidth]{figures/platform_snapshot}
	\caption{OpenVLC1.2 cape connected to the BBB board.}\label{fig_cape}
\end{figure}

\subsection{TX circuit}

The receiver's circuitry has also been modified from a OPT101 to a SFH 
206, which will allow a faster transmission rate at a much reduced cost.


Changes in the TX circuit were focused on being able to transmit faster and further. In order to do it, a new DC-DC component that support higher voltages has been introduced. With this, the LED is now feeded with 15 volts. In order to support higher state speed changes, the transistor that controls the current has also been modified for a Metal-oxide-semiconductor Field-effect transistor (MOSFET) gate driver.

\subsection{RX circuit}

In the previous version of the hardware, the bottleneck of the system was on the receiver's speed to read values from the channel. In this new version this is solved by adding a faster ADC and a new photodiode (PD). This PD, although faster and with higher range, does not amplify the signal, so external amplyfiers have been added to the receiver's circuit. The position of the PD in the board has been modified not to be shadowed by other components.

==> sec/low_view.tex <==



 







==> sec/related_work.tex <==
\section{Related work} \label{sec_related}
%\comment[Qing]{To be updated.}

We summarize the most related work to OpenVLC. 


\vspace{1mm}
\textbf{Low-end VLC systems.} Recently, a range of exciting applications have been developed with low-end VLC system: sensing human motions~\cite{Li:2015-mobicom}, interaction~\cite{Zhang:2015}, and indoor localization~\cite{Epsilon,Kuo2015}. These low-end platforms sit at the opposite extreme of high-end ({Mb/s-Gb/s}) VLC systems: they trade throughput ({Kb/s}) for cost and simplicity. 

Our system is also low-end and borrows the general idea of leveraging LEDs as receivers from~\cite{Schmid2013,giustiniano_wd}. But it differs from these previous work on two facts: i) we do not rely on a single photodetector; and ii) we do not focus solely on the simpler case of indoor scenarios with static lights. Our system provides a more flexible and reliable link to tackle challenges related to dynamic ambient light and mobility.


\vspace{1mm}
\textbf{High-end indoors.} Researchers have investigated VLC for next-generation networks with complex optical front-ends and/or sophisticated modulation methods~\cite{Zhang2015,Tsonev,Wu2014,He2015,Eroglu2015}. Most of these efforts are based on resource-rich platforms, e.g. WARP~\cite{Zhang2015,rahaim2011demonstration}, and aim at increasing data rates in point-to-point scenarios under mild lighting conditions. While most of these studies are not relevant to ours, some are orthogonal and could be used to improve the performance of our receiver. For example, in~\cite{Zhang2015}, the transmitter adjusts the transmission rate upon detecting SNR changes at the receiver, in~\cite{Eroglu2015}, multi-element transmitters are designed to improve the quality of signal distribution in a room, and in~\cite{He2015}, PDs with different FOVs are used to increase the data rate. These studies could provide a dynamic adaption of the PHY rate which is currently fixed in our work.

%\vspace{1mm}
%\textbf{High-end outdoors.} There are few VLC studies that venture outdoors. Vehicle-to-vehicle communication is an exemplary application~\cite{Liu:2011,Shun-Hsiang}. They rely mainly on simulations, but some evaluate VLC prototypes outdoors with sunlight. From these studies we learned the importance of adjusting the FOV to avoid saturation due to sunlight, particularly in~\cite{Liu:2011}. The prototypes however rely on very expensive optical front-ends such as Thorlabs-PDA100A~\cite{Shun-Hsiang}, whose cost is upwards of 300 USD. Our optical front-end is designed to operate in tiny transceivers for IoL and it costs less than 10 USD\footnote{As described before, we design two receiving chains to achieve a reliable and adaptive receiver. For the additional chain, the cost is only around 2 USD.}.
%

